Bilevel approaches for learning of variational imaging models

We review some recent learning approaches in variational imaging, based on bilevel optimisation, and emphasize the importance of their treatment in function space. The paper covers both analytical and numerical techniques. Analytically, we include results on the existence and structure of minimisers, as well as optimality conditions for their characterisation. Based on this information, Newton type methods are studied for the solution of the problems at hand, combining them with sampling techniques in case of large databases. The computational verification of the developed techniques is extensively documented, covering instances with different type of regularisers, several noise models, spatially dependent weights and large image databases.

==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-pdhgm-rho1e-05-vals.tex <==
\gdef\RESiters{1223}%
\gdef\REStime{9.9}%
\gdef\RESdist{6.626}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.706}%
\gdef\RESmu{0\ee^{+}}%
\gdef\RESgamma{0}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-05-gamma0.1-vals.tex <==
\gdef\RESiters{5}%
\gdef\REStime{24.1}%
\gdef\RESdist{11.784}%
\gdef\RESssim{0.851}%
\gdef\RESpsnr{26.705}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-05-gamma1-vals.tex <==
\gdef\RESiters{7}%
\gdef\REStime{48.2}%
\gdef\RESdist{11.701}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.766}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-05-gamma10-vals.tex <==
\gdef\RESiters{8}%
\gdef\REStime{44.0}%
\gdef\RESdist{11.703}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.765}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-05-gamma100-vals.tex <==
\gdef\RESiters{10}%
\gdef\REStime{61.6}%
\gdef\RESdist{11.704}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.764}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-08-gamma0.1-vals.tex <==
\gdef\RESiters{7}%
\gdef\REStime{36.4}%
\gdef\RESdist{6.942}%
\gdef\RESssim{0.853}%
\gdef\RESpsnr{31.301}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-08-gamma1-vals.tex <==
\gdef\RESiters{11}%
\gdef\REStime{82.3}%
\gdef\RESdist{6.656}%
\gdef\RESssim{0.894}%
\gdef\RESpsnr{31.667}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-08-gamma10-vals.tex <==
\gdef\RESiters{15}%
\gdef\REStime{86.4}%
\gdef\RESdist{6.670}%
\gdef\RESssim{0.894}%
\gdef\RESpsnr{31.648}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-08-gamma100-vals.tex <==
\gdef\RESiters{11}%
\gdef\REStime{69.0}%
\gdef\RESdist{6.673}%
\gdef\RESssim{0.894}%
\gdef\RESpsnr{31.645}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-10-gamma0.1-vals.tex <==
\gdef\RESiters{17}%
\gdef\REStime{87.9}%
\gdef\RESdist{6.940}%
\gdef\RESssim{0.853}%
\gdef\RESpsnr{31.303}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-10-gamma1-vals.tex <==
\gdef\RESiters{22}%
\gdef\REStime{165.8}%
\gdef\RESdist{6.614}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.722}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-10-gamma10-vals.tex <==
\gdef\RESiters{24}%
\gdef\REStime{141.8}%
\gdef\RESdist{6.623}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.709}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tgv2-dataset2-0.051,0.069-ssn-mu1e-10-gamma100-vals.tex <==
\gdef\RESiters{21}%
\gdef\REStime{391.6}%
\gdef\RESdist{6.625}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.707}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-pdhgm-rho1e-05-vals.tex <==
\gdef\RESiters{799}%
\gdef\REStime{2.5}%
\gdef\RESdist{6.837}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.433}%
\gdef\RESmu{0\ee^{+}}%
\gdef\RESgamma{0}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-05-gamma0.1-vals.tex <==
\gdef\RESiters{5}%
\gdef\REStime{3.4}%
\gdef\RESdist{11.784}%
\gdef\RESssim{0.851}%
\gdef\RESpsnr{26.705}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-05-gamma1-vals.tex <==
\gdef\RESiters{7}%
\gdef\REStime{6.7}%
\gdef\RESdist{11.701}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.767}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-05-gamma10-vals.tex <==
\gdef\RESiters{8}%
\gdef\REStime{6.1}%
\gdef\RESdist{11.703}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.765}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-05-gamma100-vals.tex <==
\gdef\RESiters{10}%
\gdef\REStime{7.9}%
\gdef\RESdist{11.704}%
\gdef\RESssim{0.870}%
\gdef\RESpsnr{26.764}%
\gdef\RESmu{1\ee^{-5}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-08-gamma0.1-vals.tex <==
\gdef\RESiters{6}%
\gdef\REStime{4.5}%
\gdef\RESdist{6.963}%
\gdef\RESssim{0.852}%
\gdef\RESpsnr{31.275}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-08-gamma1-vals.tex <==
\gdef\RESiters{8}%
\gdef\REStime{7.3}%
\gdef\RESdist{6.744}%
\gdef\RESssim{0.889}%
\gdef\RESpsnr{31.552}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-08-gamma10-vals.tex <==
\gdef\RESiters{9}%
\gdef\REStime{6.7}%
\gdef\RESdist{6.769}%
\gdef\RESssim{0.888}%
\gdef\RESpsnr{31.520}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-08-gamma100-vals.tex <==
\gdef\RESiters{11}%
\gdef\REStime{9.2}%
\gdef\RESdist{6.773}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.516}%
\gdef\RESmu{1\ee^{-8}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-10-gamma0.1-vals.tex <==
\gdef\RESiters{6}%
\gdef\REStime{4.0}%
\gdef\RESdist{6.960}%
\gdef\RESssim{0.852}%
\gdef\RESpsnr{31.279}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{0.1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-10-gamma1-vals.tex <==
\gdef\RESiters{8}%
\gdef\REStime{7.5}%
\gdef\RESdist{6.741}%
\gdef\RESssim{0.889}%
\gdef\RESpsnr{31.557}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{1}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-10-gamma10-vals.tex <==
\gdef\RESiters{9}%
\gdef\REStime{6.8}%
\gdef\RESdist{6.766}%
\gdef\RESssim{0.888}%
\gdef\RESpsnr{31.525}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{10}%


==> tgv-learn-resimg/COMPARE-tv-dataset2-0.051-ssn-mu1e-10-gamma100-vals.tex <==
\gdef\RESiters{11}%
\gdef\REStime{8.8}%
\gdef\RESdist{6.769}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.520}%
\gdef\RESmu{1\ee^{-10}}%
\gdef\RESgamma{100}%


==> tgv-learn-resimg/ictv-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.051}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.068}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{16}%
\gdef\RESdist{6.656}%
\gdef\RESssim{0.895}%
\gdef\RESpsnr{31.667}%
\gdef\RESerror{}%


==> tgv-learn-resimg/ictv-huberonly-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.020}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.015}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{6}%
\gdef\RESdist{8.221}%
\gdef\RESssim{0.879}%
\gdef\RESpsnr{29.832}%
\gdef\RESerror{}%


==> tgv-learn-resimg/ictv-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.041}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.051}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{6.439}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.954}%
\gdef\RESerror{}%


==> tgv-learn-resimg/ictv-l2-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.016}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.009}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{8.127}%
\gdef\RESssim{0.873}%
\gdef\RESpsnr{29.932}%
\gdef\RESerror{}%


==> tgv-learn-resimg/krtv2sketch-l2-dataset10-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.038}%
\gdef\RESalphatwo{38.806}%
\gdef\RESalphaSCtwo{2.5\ee^{+6}}%
\gdef\RESdist{38.805914}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{16}%
\gdef\RESdist{10.258}%
\gdef\RESssim{0.875}%
\gdef\RESpsnr{26.706}%
\gdef\RESerror{}%


==> tgv-learn-resimg/krtv2sketch-l2-dataset8-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.006}%
\gdef\RESalphatwo{0.421}%
\gdef\RESalphaSCtwo{2.8\ee^{+4}}%
\gdef\RESdist{0.421477}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{11}%
\gdef\RESdist{81.245}%
\gdef\RESssim{0.565}%
\gdef\RESpsnr{9.935}%
\gdef\RESerror{}%


==> tgv-learn-resimg/krtv2sketch-l2-dataset9-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.002}%
\gdef\RESalphaSCone{0.423}%
\gdef\RESalphatwo{1.4\ee^{+2}}%
\gdef\RESalphaSCtwo{9.4\ee^{+6}}%
\gdef\RESdist{144.143845}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{6}%
\gdef\RESdist{97.291}%
\gdef\RESssim{0.551}%
\gdef\RESpsnr{8.369}%
\gdef\RESerror{}%


==> tgv-learn-resimg/polytv-huberonly-dataset21-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.082}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.105}%
\gdef\RESalphathree{0.000}%
\gdef\RESalphaSCthree{0.000}%
\gdef\RESalphafour{0.001}%
\gdef\RESalphaSCfour{0.187}%
\gdef\RESdist{0.000732}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{182}%
\gdef\RESdist{14.924}%
\gdef\RESssim{0.796}%
\gdef\RESpsnr{24.653}%
\gdef\RESerror{}%


==> tgv-learn-resimg/polytv-l2-dataset21-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.040}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.089}%
\gdef\RESalphathree{0.000}%
\gdef\RESalphaSCthree{0.000}%
\gdef\RESalphafour{0.001}%
\gdef\RESalphaSCfour{0.129}%
\gdef\RESdist{0.000505}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{50}%
\gdef\RESdist{13.893}%
\gdef\RESssim{0.763}%
\gdef\RESpsnr{25.275}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-2ndhuber-dataset4-linesearch1-bfgs1-beta1e-20-uinitreg_1.000000,1.000000_-vals.tex <==
\gdef\RESalphaone{0.001441}%
\gdef\RESalphaSCone{0.37}%
\gdef\RESalphatwo{11133.045597}%
\gdef\RESalphaSCtwo{729615276.26}%
\gdef\RESdist{11133.045597}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{4}%
\gdef\RESdist{20.373}%
\gdef\RESssim{0.527}%
\gdef\RESpsnr{21.950}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.051}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.069}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{12}%
\gdef\RESdist{6.615}%
\gdef\RESssim{0.897}%
\gdef\RESpsnr{31.720}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-huberonly-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.020}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.015}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{8.236}%
\gdef\RESssim{0.879}%
\gdef\RESpsnr{29.816}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.041}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.058}%
\gdef\RESdist{0.000001}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{11}%
\gdef\RESdist{6.412}%
\gdef\RESssim{0.890}%
\gdef\RESpsnr{31.992}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-l2-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.017}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.013}%
\gdef\RESdist{0.000000}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{8}%
\gdef\RESdist{8.139}%
\gdef\RESssim{0.873}%
\gdef\RESpsnr{29.920}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-l2-dataset4-linesearch1-bfgs1-beta1e-20-uinitreg_1.000000,1.000000_-vals.tex <==
\gdef\RESalphaone{0.000065}%
\gdef\RESalphaSCone{0.02}%
\gdef\RESalphatwo{1.162246}%
\gdef\RESalphaSCtwo{76168.96}%
\gdef\RESdist{1.162246}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{8}%
\gdef\RESdist{8.182}%
\gdef\RESssim{0.871}%
\gdef\RESpsnr{29.873}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-symbregman-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.079}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{30.627}%
\gdef\RESdist{0.000467}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{35}%
\gdef\RESdist{7.845}%
\gdef\RESssim{0.877}%
\gdef\RESpsnr{30.239}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tgv2-symbregman-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.033}%
\gdef\RESalphatwo{0.000}%
\gdef\RESalphaSCtwo{0.620}%
\gdef\RESdist{0.000009}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{11}%
\gdef\RESdist{9.310}%
\gdef\RESssim{0.849}%
\gdef\RESpsnr{28.752}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-2ndhuber-dataset4-linesearch1-bfgs1-beta1e-20-uinitreg_1.000000_-vals.tex <==
\gdef\RESalphaone{0.001441}%
\gdef\RESalphaSCone{0.37}%
\gdef\RESdist{0.001441}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{4}%
\gdef\RESdist{20.373}%
\gdef\RESssim{0.527}%
\gdef\RESpsnr{21.950}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-huberonly-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.057}%
\gdef\RESdist{0.000221}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{10}%
\gdef\RESdist{6.944}%
\gdef\RESssim{0.887}%
\gdef\RESpsnr{31.298}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-huberonly-dataset21-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.234}%
\gdef\RESdist{0.000914}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{10}%
\gdef\RESdist{16.117}%
\gdef\RESssim{0.775}%
\gdef\RESpsnr{23.985}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-huberonly-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.021}%
\gdef\RESdist{0.000081}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{8.284}%
\gdef\RESssim{0.877}%
\gdef\RESpsnr{29.766}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset10-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.152}%
\gdef\RESdist{0.000592}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{5}%
\gdef\RESdist{10.405}%
\gdef\RESssim{0.882}%
\gdef\RESpsnr{26.582}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.042}%
\gdef\RESdist{0.000163}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{12}%
\gdef\RESdist{6.623}%
\gdef\RESssim{0.879}%
\gdef\RESpsnr{31.710}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset21-linesearch1-bfgs1-beta0-uinitreg_0.200000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.161}%
\gdef\RESdist{0.000628}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{5}%
\gdef\RESdist{14.689}%
\gdef\RESssim{0.739}%
\gdef\RESpsnr{24.791}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.017}%
\gdef\RESdist{0.000065}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{13}%
\gdef\RESdist{8.182}%
\gdef\RESssim{0.871}%
\gdef\RESpsnr{29.873}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset4-linesearch1-bfgs1-beta1e-20-uinitreg_1.000000_-vals.tex <==
\gdef\RESalphaone{0.000065}%
\gdef\RESalphaSCone{0.02}%
\gdef\RESdist{0.000065}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{8}%
\gdef\RESdist{8.182}%
\gdef\RESssim{0.871}%
\gdef\RESpsnr{29.873}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset8-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.001}%
\gdef\RESalphaSCone{0.311}%
\gdef\RESdist{0.001216}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{81.794}%
\gdef\RESssim{0.546}%
\gdef\RESpsnr{9.876}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-l2-dataset9-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.002}%
\gdef\RESalphaSCone{0.563}%
\gdef\RESdist{0.002199}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{7}%
\gdef\RESdist{97.205}%
\gdef\RESssim{0.552}%
\gdef\RESpsnr{8.377}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-symbregman-dataset2-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.079}%
\gdef\RESdist{0.000310}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{5}%
\gdef\RESdist{7.849}%
\gdef\RESssim{0.877}%
\gdef\RESpsnr{30.234}%
\gdef\RESerror{}%


==> tgv-learn-resimg/tv-symbregman-dataset4-linesearch1-bfgs1-beta0-uinitreg_0.100000_-vals.tex <==
\gdef\RESalphaone{0.000}%
\gdef\RESalphaSCone{0.033}%
\gdef\RESdist{0.000129}%
\gdef\RESdimX{256}%
\gdef\RESdimY{256}%
\gdef\RESiters{12}%
\gdef\RESdist{9.313}%
\gdef\RESssim{0.849}%
\gdef\RESpsnr{28.749}%
\gdef\RESerror{}%

